HVTR: Hybrid Volumetric-Textural Rendering for Human Avatars

We propose a novel neural rendering pipeline, Hybrid Volumetric-Textural Rendering (HVTR), which synthesizes virtual human avatars from arbitrary poses efficiently and at high quality. First, we learn to encode articulated human motions on a dense UV manifold of the human body surface. To handle complicated motions (e.g., self-occlusions), we then leverage the encoded information on the UV manifold to construct a 3D volumetric representation based on a dynamic pose-conditioned neural radiance field. While this allows us to represent 3D geometry with changing topology, volumetric rendering is computationally heavy. Hence we employ only a rough volumetric representation using a pose-conditioned downsampled neural radiance field (PD-NeRF), which we can render efficiently at low resolutions. In addition, we learn 2D textural features that are fused with rendered volumetric features in image space. The key advantage of our approach is that we can then convert the fused features into a high-resolution, high-quality avatar by a fast GAN-based textural renderer. We demonstrate that hybrid rendering enables HVTR to handle complicated motions, render high-quality avatars under user-controlled poses/shapes and even loose clothing, and most importantly, be efficient at inference time. Our experimental results also demonstrate state-of-the-art quantitative results.

==> sec/X_supplementary_copy.tex <==

\begingroup
\renewcommand{\arraystretch}{1.25}
\begin{table}[th]
	\centering
	\begin{tabular}{cl}
		\hline
		Term                       & Description                                      \\ \hline \hline
		$M_P$                       & Input SMPL mesh                                  \\
		$o$, $d$                        & Target viewpoint (camera position and direction) \\
		$I_{t}$               & Rendered target image                            \\ \hline \hline
		$F_N$                       & NormalNet (network)                              \\
		$F_P$                       & PoseNet (network)                                \\
		$F_R$                       & TexRenderer (network)                            \\
		$F_T$                       & Texture Encoder (network)                        \\
		$F_\theta$                       & MLPs of PD-NeRF (network)                        \\
		$Z_G$                       & Optimizable Geometry Latent                      \\
		$Z_T$                       & Optimizable Texture Latent                       \\ \hline \hline
		$\Psi^{uv}_{N}$  & Normal of SMPL mesh in UV space           \\
		$\Psi^{uv}_{P}$  & Stacked pose-dependent featuers in UV space      \\
		$\Psi^{3D}_{P}$ & Features of PD-NeRF in 3D space                  \\
		$\Psi^{im}_{P}$ & Pose-dependent neural textures in image space    \\
		$\Psi^{im}_{tex}$ & Extracted textural features in image space       \\
		$\Psi^{im}_{vol}$ & Rasterized volumetric features in image space    \\
		$\Psi^{im}_{uv}$ & UV coordinate map in image space   \\ \hline            
	\end{tabular}
	\caption{Glossary table. Terms we used in the paper.}
	\label{tab:term_table}
\end{table}
\endgroup

\section{More Experimental Results}
\subsection{Comparisons}

\noindent \textbf{Free-Viewpoint Synthesis.} We evaluate the results of image synthesis under novel views on ZJU\_MoCap \cite{neuralbody} dataset by following the same protocol as Neural Body \cite{neuralbody}, as shown in Fig.~\ref{fig:free_view_nb}. The ZJU\_MoCap \cite{neuralbody} dataset was captured in a studio with uneven lighting, which disturbs the learning of wrinkles, and affect the quantitative evaluations. In addition, the sequences of ZJU\_MoCap are generally short (about 800 frames in average for each camera) with small pose variations. Hence, the ZJU\_MoCap datasets are mainly used to evaluate the capability of rendering high-frequency details instead of pose generalization, and this is also why they were not widely used in the follow-up animation related papers (e.g., \cite{neuralactor,Peng2021AnimatableNR}).

\begin{table*}[th]\small
	\begin{minipage}{\linewidth}		
		\begin{center}
			%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
			\includegraphics[width=\linewidth]{img/free_view_nb.PNG}
		\end{center}
	\end{minipage}
	\begin{minipage}{.48\linewidth}
		\begin{center}
			\begin{tabular}{ccccc}
				\hline
				Z1 (this example)  & LPIPS $\downarrow$ & FID $\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$\\ \hline
				Neural Body \cite{neuralbody}  & .153          & 90.74          & \textbf{.886}          & \textbf{26.51}          \\
				Ours & \textbf{.112} & \textbf{56.94} & {.855} & {23.75} \\ \hline \hline
				\textbf{Z1 (mean)} & LPIPS $\downarrow$ & FID $\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$\\ \hline
				Neural Body \cite{neuralbody}  & .137          & 120.73          & \textbf{.889}          & {\textbf{29.09}}          \\
				Ours & \textbf{.117} & \textbf{87.55} & {.853} & {26.16} \\ \hline
			\end{tabular}
			%\captionof{table}{Comparisons with AniNeRF on R1 dataset under novel poses. }
			%\label{tab:aninerf}
		\end{center}
	\end{minipage}
	\hfill
	\begin{minipage}{.48\linewidth}
		\begin{center}
			\begin{tabular}{ccccc}
				\hline
				Z3 (this example)  & LPIPS  & FID  & SSIM & PSNR\\ \hline 
				Neural Body \cite{neuralbody}  & .170          & 112.70          & \textbf{.866}          & \textbf{26.16}          \\
				Ours & \textbf{.124} & \textbf{52.23} & {.816} & {22.09} \\ \hline \hline
				\textbf{Z3 (mean)} & LPIPS  & FID  & SSIM & PSNR\\ \hline
				Neural Body \cite{neuralbody}  & .149          & 132.05          & \textbf{.872}          & \textbf{26.35}          \\
				Ours & \textbf{.098} & \textbf{69.79} & {.848} & {24.08} \\ \hline
			\end{tabular}
			%\captionof{table}{Comparisons with AniNeRF on R1 dataset under novel poses. }
			%\label{tab:aninerf}
		\end{center}
	\end{minipage}
	\captionof{figure}{We evaluate the results of image synthesis on novel views while the test poses are the same as training poses,  by following the same protocol as Neural Body \cite{neuralbody} on Z1 and Z3 sequences from ZJU\_MoCap \cite{neuralbody} dataset (see more details in the paper). Both methods are trained on 4 cameras, and evaluated on the hold-out cameras. Our synthesized results recover more details, and significantly outperform Neural Body on LPIPS \cite{lpip} and FID \cite{Heusel2017GANsTB}.  The ZJU\_MoCap dataset suffers from uneven lighting, and both Neural Body and ours cannot recover the right lighting. Yet in this case, the LPIPS and FID capture human judgement better than per-pixel metrics such as SSIM \cite{ssim} or PSNR, as stated in  \cite{lpip}.}
	\label{fig:free_view_nb} 
\end{table*}


\noindent \textbf{Forward vs. Backward Skinning}. AniNeRF \cite{Peng2021AnimatableNR} parameterizes clothes with skinning weights by learning backward skinning, which generally requires a large training dataset, and cannot solve one-to-many backward correspondences \cite{Chen2021SNARFDF} shown in Fig. \ref{fig:cmp_ani}, whereas we only need a forward skinning step and avoid the multi-correspondence problem. The experiment on R1 dataset shows that our method significantly outperforms AniNeRF on all the four metrics in Tab. \ref{tab:aninerf}, where the same protocol as Tab. \ref{tab:quan_all} is used for training and testing.


\begin{table}
	\begin{minipage}{\linewidth}
		\begin{center}
			\includegraphics[width=.8\linewidth]{img/cmp_ani_nerf.png}
			\captionof{figure}{Comparisons of backward skinning method (AniNeRF \cite{Peng2021AnimatableNR}) and forward skinning method (ours).  AniNeRF suffers from artificats since it cannot solve the one-to-many backward correspondence problem.}
			%	\vspace{-0.1in}
			\label{fig:cmp_ani}
		\end{center}
	\end{minipage}

	\vspace{0.1in}
	\hfill
	
	\begin{minipage}{\linewidth}
		\begin{center}
			\begin{tabular}{ccccc}
				\hline
				& LPIPS $\downarrow$ & FID $\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$\\ \hline
				AniNeRF \cite{Peng2021AnimatableNR}  & .271          & 196.44          & .773          & 23.36          \\
				Ours & \textbf{.090} & \textbf{62.33} & \textbf{.842} & \textbf{26.22} \\ \hline
			\end{tabular}
			\captionof{table}{Comparisons with AniNeRF on R1 dataset under novel poses. }
			\label{tab:aninerf}
		\end{center}
	\end{minipage}
\end{table}

\noindent \textbf{Qualitative Comparisons on R5, R6, and Z2 Dataset.}
The qualitative comparisons on R5, R6, and Z2 are shown in Fig.~\ref{fig:otherhuman}. %Note that Neural Body \cite{neuralbody} cannot converge to a detailed generation as seen in Fig.~\ref{fig:nb_converge}.

\noindent \textbf{Accuracy and Inference Time.}
The accuracy and inference time of each method are shown in Tab.~\ref{tab:full_acc_time_supp}.

\noindent \textbf{GPU Memory.} Ours\_4(20)-most GPU-consuming version: 21GB; Neural Body: 5GB; ANR:11GB. Note that we need much GPU memory in training, because HVTR renders a full image of PD-NeRF at each iteration, whereas Neural Body just randomly sample points to calculate gradients.  However, in inference, Ours\_4(20): 4GB, Neural Body: 15GB. Note that this was evaluated on the cropped bbox with downsampled \textit{\textbf{S=4}}, and we can process high resolution like $1024\times1024$ (Z1-3) or $1285\times940$ (M1).

\noindent \textbf{Shape Editing.} See the right figure, where ours generate high-quality faces \cnum{1}\cnum{2} and wrinkles \cnum{3}\cnum{4} and shapes \cnum{5}. Ours disentangles body and clothes better \cnum{3} than SMPLpix \cite{smplpix}. We will provide video comparisons in the revised version.

\begin{table*}

	\begin{minipage}{.5\linewidth}
		%\vspace{-0.12in}
		\begin{center}
			%\vspace{-0.16in}
			\includegraphics[width=\linewidth]{img/ab.jpg}
			%\vspace{-0.3in}
			%\caption{Ablation study.}
			%\vspace{-0.3in}
			%\label{fig:ab}
		\end{center}    
	\end{minipage}
	
	\hfill

	\begin{minipage}{.5\linewidth}
		%\vspace{-0.1in}
		%\small
		\begin{center}
			\begin{tabular}{lcccc}
				\hline
				& LPIPS $\downarrow$ & FID $\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$\\ \hline
				w/o D       & 1.210  & 87.533 & \textbf{.850} & \textbf{26.863} \\
				w/o $F_P$   & .955  & 67.613 & .838 & 26.167 \\
				w/o $F_N$   & .927  & 65.310 & .839 & 26.295 \\
				w/o $F_T$   & .970  & 69.063 & .835 & 26.027 \\
				w/o $Z_G$   & .904  & 63.114 & .843 & 26.310 \\            
				Ours        & \textbf{.901}  & \textbf{62.333} & .842 & 26.217 \\ \hline
			\end{tabular}
			%\vspace{-0.1in}
			\captionof{figure}{Ablation under the same setting as Tab. 4. LPIPS and FID capture human judgement better than per-pixel SSIM/PSNR (higher for blurry `w/o D'). LPIPS $\times10$ shown.}
			\label{fig:ab}
			%\vspace{-0.34in}
		\end{center}    
	
	\end{minipage}
\end{table*}







\begin{figure}[ht]
	\begin{center}
		%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
		\includegraphics[width=\linewidth]{img/shape_editing_NB_SMPLpix.png}
	\end{center}
	\caption{Comparisons of method trained with or without face identity loss. Ours(-F) indicates a variant of our method that is not trained with face identity loss.}
	\label{fig:shapeedit_comp}
\end{figure}


\subsection{Ablation Study}
\noindent \textbf{Face Identity Loss}. We use the face identity loss to improve the qualitative results as shown in Fig.~\ref{fig:face} (also used in \cite{egorend,feanet}), whereas the improvements of faces do not improve the overall quantitative results of each method, as listed in Tab.~\ref{tab:face_loss}.

\begin{figure*}[ht]
	\begin{center}
		%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
		\includegraphics[width=.8\linewidth]{img/face_identity.jpg}
	\end{center}
	\caption{Comparisons of method trained with or without face identity loss. Ours(-F) indicates a variant of our method that is not trained with face identity loss.}
	\label{fig:face}
\end{figure*}


\begin{table}
	\centering
	\begin{tabular}{lcccc}
		\hline
		\textbf{R3} & LPIPS $\downarrow$ & FID $\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$\\ \hline
		DNR	&.108	& 80.33	&.809	&24.05 \\
		DNR + F	&\textbf{.103}	&\textbf{75.42}	&\textbf{.812}	&\textbf{24.13} \\ \hline
		
		SMPLPix	&\textbf{.104}	&\textbf{74.57}	&.810	&\textbf{24.16} \\
		SMPLPix + F	&.109	&78.59	&\textbf{.811}	&23.93 \\ \hline \hline
		
		\textbf{R2} & LPIPS $\downarrow$ & FID $\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$\\ \hline
		DNR	& .128	& 105.63	& \textbf{.820}	& 27.82 \\
		DNR + F	& \textbf{.125}	& \textbf{98.86}	& \textbf{.820}	& \textbf{27.92} \\ \hline
		
		SMPLPix	&\textbf{.124}	&99.81	&.822	& 27.92 \\
		SMPLPix + F	&\textbf{.124}	&\textbf{94.81}	&\textbf{.826}	& \textbf{27.97} \\ \hline \hline
		
		\textbf{R1} & LPIPS $\downarrow$ & FID $\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$\\ \hline
		DNR	& \textbf{.102}	& \textbf{75.02}	& .831	& 25.73 \\
		DNR + F &	.103 &	75.35 &	\textbf{.832} &	\textbf{25.85} \\ \hline
		
		SMPLPix	& \textbf{.100}	& \textbf{69.81}	& \textbf{.835}	& \textbf{25.93} \\
		SMPLPix + F	& .104	& 75.34	& .833	& 25.81 \\ \hline
		
		Ours(-F)	& \textbf{.088}	& \textbf{61.03}	& .841	& \textbf{26.42} \\
		Ours	&.090	& 62.33	& \textbf{.842}	& 26.22 \\ \hline
	\end{tabular}
	\caption{Quantitative results of each method trained with or without face identity loss. Ours(-F) indicates a variant of our method that is not trained with face identity loss. (DNR + F) and (SMPLpix + F) are trained with face identity loss.}
	\label{tab:face_loss}
	%\vspace{-0.12in}	
\end{table}	

\noindent \textbf{Feature Fusion}. We compare two methods to fuse the volumetric and textural features as discussed at Sec. 3.3 by concatenation (Concat) and Attentional Feature Fusion (AFF \cite{dai21aff}) on two datasets, R1 and R2 (about 12K frames in training, 3K frames in testing) in Tab.~\ref{tab:feat_fusion}, which show that AFF can improve the LPIPS \cite{lpip} and FID \cite{Heusel2017GANsTB} results.

\begin{table}
	\begin{center}			
		\begin{tabular}{ccccc}
			\hline
			\textbf{R2} & LPIPS $\downarrow$ & FID $\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$\\ \hline
			Concat  & .117          & 90.43          & \textbf{.838}          & {28.55}          \\
			AFF & \textbf{.108} & \textbf{84.43} & {.833} & \textbf{28.62} \\ \hline
			\hline
			\textbf{R1} & LPIPS $\downarrow$ & FID $\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$\\ \hline
			Concat  & .099          & 64.54          & \textbf{.856}          & \textbf{26.78}          \\
			AFF & \textbf{.090} & \textbf{62.33} & {.842} & {26.22} \\ \hline
		\end{tabular}
	\end{center}
	\vspace{-0.12in}
		\caption{Comparisons of fusing volumetric and textural features by concatenation (Concat) and Attentional Feature Fusion (AFF \cite{dai21aff}) on R1 and R2 dataset.}
		\label{tab:feat_fusion}
	\end{table} 

% \begin{table}
% 	\begin{center}
% 	\begin{tabular}{lcccc}
% 		\hline
% 		M1   & LPIPS $\downarrow$ & FID $\downarrow$ & SSIM$\uparrow$ & PSNR$\uparrow$\\ \hline
% 		DNR  & .195          & 144.78          & .687          & 19.96          \\
% 		Ours & \textbf{.179} & \textbf{132.83} & \textbf{.696} & \textbf{20.18} \\ \hline
% 	\end{tabular}
% 	\end{center}
% 	\vspace{-0.06in}
% 	\caption{Quantitative results on M1 dataset under novel poses and views. Qualitative results are shown in Fig. 5 of the main paper. }
% 	\label{tab:quan_dress}
% 	\vspace{-0.2in}
% \end{table}

\begin{table*}[th]
	\begin{minipage}{.48\linewidth}		
		\begin{center}
			%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
			\includegraphics[width=.9\linewidth]{img/dilation_2.png}
		\end{center}
		\vspace{-0.12in}
		\captionof{figure}{Right: Geometry-guided ray marching. Left: sampling points by SMPL mesh dilation. Red - SMPL model; Gray - rays and sampled points.}
		\label{fig:dilation}
		%\vspace{-0.3in}		
	\end{minipage}
	\hfill
	\begin{minipage}{.48\linewidth}
		%\vspace{-0.06in}
		\begin{center}
			%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
			\includegraphics[width=\linewidth]{img/geometry.png}
		\end{center}
		%\vspace{-0.1in}
		\captionof{figure}{Construct PD-NeRF with $45\times45$ resolution images and 7 sampled point along each ray: left (geometry), right (reference image).}
		\label{fig:geo45}
		%\vspace{-0.1in}
	\end{minipage} 
\end{table*}

\begin{table*}[t]\small
    \centering
	\begin{tabular}{lcccccccccccc}
		\hline
		& \multicolumn{4}{l}{R1}                                          & \multicolumn{4}{l}{R2}                                          & \multicolumn{4}{l}{R3}                                          \\ \hline
		Models      & LPIPS$\downarrow$         & FID$\downarrow$            & SSIM$\uparrow$          & PSNR$\uparrow$           & LPIPS        & FID            & SSIM          & PSNR           & LPIPS         & FID            & SSIM          & PSNR           \\ \hline 
		DNR         & .102          & 75.02          & .831          & 25.73          & .125          & 98.86          & .820          & 27.92          & .108          & 80.33          & .809          & 24.05          \\
		SMpix     & .100          & 69.81          & .835          & 25.93          & .124          & 94.81          & .826          & 27.97          & .104          & 74.57          & .810          & 24.16          \\
		ANR         & .117          & 78.50          & .830          & 26.02          & .129          & 101.72         & .825          & 28.30          & .098          & 69.14          & .813          & 24.29          \\
		NB & .212          & 155.84         & .833          & 26.17          & .218          & 161.99         & \textbf{.833} & 28.61          & .240          & 165.03         & .811          & 24.16          \\
		Ours        & \textbf{.090} & \textbf{62.33} & \textbf{.842} & \textbf{26.22} & \textbf{.108} & \textbf{84.43} & \textbf{.833}          & \textbf{28.62} & \textbf{.093} & \textbf{66.01} & \textbf{.823} & \textbf{24.55} \\
		\hline \hline
		& \multicolumn{4}{l}{R4}                                          & \multicolumn{4}{l}{R5}                                          & \multicolumn{4}{l}{R6}                                          \\
		\hline
		DNR         & .108          & 93.16          & .833          & 23.34          & .136          & 121.50         & .817          & 24.06          & .088          & 74.77          & .864          & 25.81          \\
		SMpix     & .107          & 88.14          & .837          & 23.37          & .131          & 118.64         & .818          & 24.10          & .077          & 64.33          & .875          & 26.14          \\
		ANR         & .138          & 91.92          & .812          & 23.26          & .140          & 123.55         & .823          & 24.67          & .083          & 63.16          & .875          & 26.61          \\
		NB & .198          & 126.26         & \textbf{.856} & \textbf{24.26} & .220          & 161.93         & .816          & 24.25          & .142          & 94.96          & .880          & 27.19          \\
		Ours        & \textbf{.096} & \textbf{78.79} & .849          & 23.98          & \textbf{.117} & \textbf{93.56} & \textbf{.827} & \textbf{24.84} & \textbf{.070} & \textbf{57.00} & \textbf{.891} & \textbf{27.42} \\ \hline \hline
		& \multicolumn{4}{l}{Z1}                                          & \multicolumn{4}{l}{Z2}                                          & \multicolumn{4}{l}{Z3}                                          \\ \hline
		DNR         & .145          & 92.78          & .797          & 22.06          & .145          & 87.27          & .774          & 25.04          & .109          & 82.79          & .826          & 23.16          \\
		SMpix     & .150          & 90.90          & .797          & 22.14          & .144          & 81.78          & .774          & 25.18          & .113          & 83.96          & .827          & 22.92          \\
		ANR         & .205          & 171.69         & .775          & \textbf{22.35}          & .159          & 110.85         & .778          & 25.41          & .173          & 123.84         & .790          & 22.14          \\
		NB & .215          & 163.83         & .789          & 22.16          & .238          & 155.27         & \textbf{.792}          & \textbf{25.88}          & .204          & 167.66         & .825          & \textbf{23.89} \\
		Ours        & \textbf{.143} & \textbf{90.43} & \textbf{.805} & {22.31} & \textbf{.132} & \textbf{79.14} & {.785} & {25.69} & \textbf{.105} & \textbf{78.03} & \textbf{.829} & 23.23          \\ \hline 
	\end{tabular}
	\vspace{0.02in}
	\caption{Quantitative comparisons on nine sequences (averaged on all test views and poses). SMpix: SMPLpix, NB: Neural Body. To reduce the influence of the background, all scores are calculated from images cropped to 2D bounding boxes. LPIPS \cite{lpip} and FID \cite{Heusel2017GANsTB} capture human judgement better than per-pixel metrics such as SSIM \cite{ssim} or PSNR. All poses are novel, and R4, Z1-Z3 are tested on new views.} %whereas the pose generalization is not obvious
	%\vspace{-0.1in}
	\label{tab:quan_all}
\end{table*}

%\begin{figure}[h]
%	\begin{center}
		%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%		\includegraphics[width=\linewidth]{img/nb_converge.png}
%	\end{center}
%	\caption{Convergence of Neural Body in training. Left: training results of one frame after 100,000 iterations; Middle: after 150,000 iterations; Right: ground truth.}
%	\label{fig:nb_converge}
%\end{figure}

\section{Implementation Details}
\noindent \textbf{Optimization}. The networks were trained using the Adam optimizer \cite{adam} with an initial learning rate of $2\times 10^{-4}$, $\beta_1 = 0.5$. The loss weights \{$\lambda_{vol}$, $\lambda_{norm}$, $\lambda_{feat}$, $\lambda_{mask}$, $\lambda_{pix}$, $\lambda_{adv}$, $\lambda_{face}$\} are set empirically to $\{15,1,10,5,1,1,5\}$. We train DNR\cite{dnr}, SMPLpix\cite{smplpix}, ANR\cite{anr}, and our method for 50,000 iterations, and 180,000 iterations for Neural Body \cite{neuralbody}, and 250,000 iterations for Animatable NeRF (AniNeRF \cite{Peng2021AnimatableNR}). We train the networks with a Nvidia P6000 GPU, and it generally takes 28 hours for DNR and SMPLpix, and 40 hours for our method. Note that Neural Body \cite{neuralbody} can only converge to averaged and blurry results (Fig.~\ref{fig:nb_converge}) even in training stage especially on long sequences, which is also stated in \cite{neuralactor}.

\noindent \textbf{Network Architectures and Optimizable Latents}. $Z_G$ and $Z_T$ both have a size of $128 \times 128 \times 16$. $\bigs{F_P}$ is based on Pix2PixHD \cite{pix2pixhd} architecture with Encoder blocks of [Conv2d, Batch- Norm, ReLU], ResNet \cite{He2016DeepRL} blocks, and Decoder blocks of [ReLU, ConvTranspose2d, BatchNorm]. $\bigs{F_P}$ has 3 Encoder and Decode blocks, and 2 ResNet blocks. $\bigs{F_N}$ has 2 Decode blocks. $\bigs{F_T}$ has $n$  ($n$ = 2 or 3 or 4) Encoder blocks, and the exact number depends on the downsampling factor of PD-NeRF such that the textural features and volumetric features have the same size as discussed at Sec. 3.4. $\bigs{F_R}$ has (${4-n}$) Encoder blocks, 4 Decoder blocks, and 5 ResNet blocks. For $\bigs{F_{\theta}}$, we use an 7-layer MLP with a skip connection from the input to the 4th layer as in DeepSDF \cite{park2019deepsdf}. From the 5th layer, the network branches out two heads, one to predict density with one fully-connected layer and the other one to predict color features with two fully-connected layers.

\begin{table*}[t]

	\begin{minipage}{\linewidth}
		\centering
		\begin{tabular}{lcccccc}
			\hline
			Models       & \multicolumn{1}{l}{LPIPS$\downarrow$} & \multicolumn{1}{c}{FID$\downarrow$} & \multicolumn{1}{c}{SSIM $\uparrow$} & \multicolumn{1}{c}{PSNR$\uparrow$} & \multicolumn{1}{c}{Time (s)} & \multicolumn{1}{c}{VR\_T(\%)} \\ \hline
			DNR          & 0.1023                    & 75.0152                 & 0.8310                   & 25.7303                  & 0.184                        & -                            \\
			SMPLpix      & 0.1002                    & 69.8119                 & 0.8350                   & 25.9295                  & 0.198                        & -                            \\
			ANR          & 0.1172                    & 78.5012                 & 0.8301                   & 26.0168                  & 0.224                        & -                            \\
			Neuray Body  & 0.2124                    & 155.8382                & 0.8328                   & 26.1718                  & 18.200                       & -                            \\
			Ours\_16(7)  & 0.0966                    & 64.8711                 & \textbf{0.8489}          & \textbf{26.4356}         & 0.292                        & 11.99                        \\
			Ours\_16(12) & 0.0911                    & 64.0892                 & 0.8417                   & 26.3272                  & 0.295                        & 12.88                        \\
			Ours\_16(20) & 0.0905                    & 62.8823                 & 0.8412                   & 26.3423         & 0.305                        & 15.41                        \\
			Ours\_8(12)  & 0.0901                    & 62.3330                 & 0.8415                   & 26.2165                  & 0.349                        & 26.36                        \\
			Ours\_4(20)  & \textbf{0.0861}           & \textbf{60.7884}        & 0.8461                   & 26.2465                  & 0.464                        & 44.61                        \\ \hline		
		\end{tabular}
		\caption{Performance, inference time of each methods. VR\_T(\%) indicates the percentages of the volume rendering time. Compared with Tab.~4 of the paper, the other two metrics SSIM and PSNR are included.}
		\label{tab:full_acc_time_supp}
	\end{minipage}
	
	\vspace{0.1in}

	\hfill
	
	\begin{minipage}{\linewidth}
		\begin{center}
			%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
			\includegraphics[width=.95\linewidth]{img/otherhuman.png}
		\end{center}
		\captionof{figure}{Qualitative comparisons on R5, R6, and Z2 Dataset.}
		\label{fig:otherhuman}
	\end{minipage}
\end{table*}	


\noindent \textbf{Geometry-guided Ray Marching}. The success of our method depends on the efficient and effective training of the pose-conditioned downsampled NeRF (PD-NeRF). First, instead of sampling rays in the whole space, we utilize a geometry-guided ray marching mesh as illustrated in Fig.~\ref{fig:dilation}. Specifically, we only sample query points along the corresponding rays near the SMPL \cite{smpl} mesh surface, which is determined by a dilated SMPL mesh. The SMPL mesh is dilated along the normal of each face with a radius of $d$, where $d$ is about 12cm for general clothes and 20cm for loose clothing like skirts for M1 dataset (see Fig.~5 of the paper). We find the near and far points by querying the Z-buffer of the corresponding pixels after projecting the dilated SMPL mesh using Pytorch3D \cite{ravi2020pytorch3d}. In addition, we sample more points to the near region, which is expected to contain visible contents. The geometry-guided ray marching algorithm and UV conditioned architecture enable us to train a PD-NeRF with $45\times45$ resolution images and only 7 sampled point along each ray, as shown in Fig.~\ref{fig:geo45}. Though learned from low resolution images, the reconstructed geometry still preserves some pose-dependent features.



